Neural Architectures for Fine-grained Entity Type Classification

In this work, we investigate several neural network architectures for fine-grained entity type classification. Particularly, we consider extensions to a recently proposed attentive neural architecture and make three key contributions. Previous work on attentive neural architectures do not consider hand-crafted features, we combine learnt and hand-crafted features and observe that they complement each other. Additionally, through quantitative analysis we establish that the attention mechanism is capable of learning to attend over syntactic heads and the phrase containing the mention, where both are known strong hand-crafted features for our task. We enable parameter sharing through a hierarchical label encoding method, that in low-dimensional projections show clear clusters for each type hierarchy. Lastly, despite using the same evaluation dataset, the literature frequently compare models trained using different data. We establish that the choice of training data has a drastic impact on performance, with decreases by as much as 9.85% loose micro F1 score for a previously proposed method. Despite this, our best model achieves state-of-the-art results with 75.36% loose micro F1 score on the well- established FIGER (GOLD) dataset.

==> GNUmakefile <==
# GNU Makefile for LaTeX projects (papers, presentations, etc.), works fine
#	for projects where each TeX-file is self-contained (usually the case).
#
# Note: We assume that each TeX-file depends on all images and Bib-files, this
# 	is not ideal but is the safest choice unless you know a way to extract
# 	this information for the TeX-files (do tell me if you do, but I doubt it
# 	since TeX is Turing complete last time I checked).
#
# Author:		Pontus Stenetorp	<pontus stenetorp se>
# Version:		2013-05-14

TEX_FILES=figer.tex
TEX_BNAMES=${subst .tex,,${TEX_FILES}}
PDF_FILES=${subst .tex,.pdf,${TEX_FILES}}
BIB_FILES=${shell find -maxdepth 1 -name '*.bib' | xargs -n 1 -r basename}

LATEX_BIN=pdflatex
BIBSORT_SH=~/git/ppod/ext/bibsort/bibsort

# Drop your images into this directory (we do try to handle any necessary
# 	conversions).
IMAGE_DIR=images
SVG_IMAGES=${shell find '${IMAGE_DIR}' -name '*.svg'}
PDF_IMAGES=${subst .svg,.pdf,${SVG_IMAGES}}

# Goal(s) for converting SVG to PDF using Inkscape.
define svg2pdf-target
${2}: ${1}
	inkscape -z --file='${1}' --export-pdf='${2}' -D
endef
${foreach SVG_IMAGE,${SVG_IMAGES}, \
	${eval ${call svg2pdf-target,${SVG_IMAGE}, \
		${subst .svg,.pdf,${SVG_IMAGE}}} \
	} \
}

# Goal(s) for generating our final PDFs.
define pdf-target
${1}.blg: ${1}.tex ${BIB_FILES} ${PDF_IMAGES}
	${LATEX_BIN} '${1}'
	if grep '\\bibcite' '${1}.aux' || grep '\\citation' '${1}.aux'; \
	then \
		for _ in `seq 2`; \
		do \
			bibtex '${1}'; \
		done; \
	fi

${1}.pdf: ${1}.blg
	${LATEX_BIN} '${1}'
	for _ in `seq 2`; \
	do \
		if grep -i 'rerun' '${1}.log'; \
		then \
			${LATEX_BIN} '${1}.tex'; \
		fi; \
	done
endef
${foreach TEX_BNAME,${TEX_BNAMES}, \
	${eval ${call pdf-target,${TEX_BNAME}} \
	} \
}

.DEFAULT_GOAL=all
all: ${PDF_FILES}

# XXX: Not done...
#.PHONY: bibsort
#bibsort:
#trap "rm -f $${TMP}" INT TERM EXIT
#	find . -maxdepth 1 -name '*.bib' -exec sh -c \
#		"TMP=`mktemp` && cat {} | ${BIBSORT_SH} > $${TMP} && cat $${TMP} > {} && rm -f $${TMP}" \;
# TMP=`mktemp`; trap "rm -f ${TMP}" INT TERM EXIT; cat sture.bib | ~/git/ppod/ext/bibsort/bibsort > ${TMP}; cat ${TMP} > sture.bib; rm -f ${TMP}

.PHONY: clean
clean:
	for TEX_BNAME in ${TEX_BNAMES}; \
	do \
		for SUFFIX in aux bbl blg dvi idx lof log lot nav out pdf ps snm toc; \
		do \
			rm -f "$${TEX_BNAME}.$${SUFFIX}"; \
		done; \
	done
	rm -f ${PDF_IMAGES}
	find . -maxdepth 1 -name '*~' | xargs -r rm

